TRILLsson: Distilled Universal Paralinguistic Speech Representations

Recent advances in self-supervision have dramatically improved the quality of speech representations. However, deployment of state-of-the-art embedding models on devices has been restricted due to their limited public availability and large resource footprint. Our work addresses these issues by publicly releasing a collection of paralinguistic speech models that are small and near state-of-the-art performance. Our approach is based on knowledge distillation, and our models are distilled on public data only. We explore different architectures and thoroughly evaluate our models on the Non-Semantic Speech (NOSS) benchmark. Our largest distilled model is less than 15% the size of the original model (314MB vs 2.2GB), achieves over 96% the accuracy on 6 of 7 tasks, and is trained on 6.5% the data. The smallest model is 1% in size (22MB) and achieves over 90% the accuracy on 6 of 7 tasks. Our models outperform the open source Wav2Vec 2.0 model on 6 of 7 tasks, and our smallest model outperforms the open source Wav2Vec 2.0 on both emotion recognition tasks despite being 7% the size.

==> table_ablation.tex <==
\begin{table}[!t]
\captionsetup{size=footnotesize}
\centering
\caption{Ablation studies.}\label{tab:ablation}
\footnotesize
\begin{tabular}{r | c c c } \toprule
  Ablation & Avg Decrease & Std &  N  \\
  \midrule
  Local $->$ Global matching & 0.9\% & 0.8 & ?  \\
  3 sec $->$ 2 sec & ? & ? & ?  \\
  LL only & ? & ? & ? \\
  AS only & ? & ? & ? \\
 \bottomrule
\end{tabular}
\end{table}
%\vspace{-5em}

==> table_model_hparams.tex <==
\begin{table}[!t]
\captionsetup{size=footnotesize}
\centering
\caption{Model hyparameters. Most but not all combinations are valid, so ``total models" isn't a strict carteisian product of the hparams.}\label{tab:train_hp}
\footnotesize
\begin{tabular}{r r l } \toprule
  Architecture & Hyperparameter & Values \\
  \midrule
  \textbf{AST} & Depths  & 4, 6, 12, 24 \\
               & Filter width & 512, 1024, 2048 \\
               & Chunk size (s)  & 2, 3 \\
               & Target matching  & local, global \\
               & \textbf{Total models} & 56 \\
  
  \midrule
  \textbf{EfficientNet} & Version & 1, 2 \\
               & Size    & 0-6/7 \\
               & Chunk size (s)  & 2, 3 \\
               & Target matching  & local, global \\
               & \textbf{Total models} & 60 \\
               \midrule
  \textbf{Resnetish} & Depths  & 8-12\\
        & Filter scale  & 1.0, .75, 0.5, .25 \\
        & Chunk size (s)  & 2, 3 \\
        & Target matching  & local, global \\
  & \textbf{Total models} & 20 \\
 \bottomrule
\end{tabular}
\end{table}
%\vspace{-5em}

==> table_results_v1.tex <==
\begin{centering}
\begin{table*}[t]
\scriptsize
\vspace{-0.2cm}
%\caption{Accuracies (\%) for NOSS tasks. }
\caption{Test performance on the NOSS Benchmark and extended tasks. ``Prev SoTA" are arbitrarily complicated models, but \textbf{all other rows are linear models on time-averaged input}.
$^\dagger$We use a filtered subset of Voxceleb1 according to YouTube’s privacy guidelines. We omit previous SoTA results on this dataset, since they used the entire dataset.
$^\ddagger$The Masked Speech task performance is reported using unweighted average recall~\cite{compare2020} instead of accuracy. Also, test set labels are not available, so we report accuracy on the eval set. 
$^{**}$ASVSpoof uses equal error rate~\cite{asvspoof}.
$^{\#}$Euphonia is the only non-public dataset. We exclude it from aggregate scores.
}\label{tab:results}

\centering
\begin{tabular}{@{} llcc|ccccccccc @{}}
\toprule[2pt]
\begin{tabular}{@{}c@{}}Model\\(input)\end{tabular} &
Arch. &
\begin{tabular}{@{}c@{}}Params\\ (M)\end{tabular} &
\begin{tabular}{@{}c@{}}Size\\ (MB)\end{tabular} &
\begin{tabular}{@{}c@{}}Avg D-\\ Prime\end{tabular}   & 
Voxceleb1$^\dagger$ & 
Voxforge & 
\begin{tabular}{@{}c@{}}Speech \\ Commands\end{tabular}   &  
\begin{tabular}{@{}c@{}}Masked \\ Speech$^\ddagger$\end{tabular}  & 
\begin{tabular}{@{}c@{}}ASVSpoof\\ 2019$^{**}$\end{tabular} & 
Euphonia$^{\#}$ &
CREMA-D &
IEMOCAP
\\
\toprule[2pt]
\textbf{Prev SoTA}
& -
& -
& -
& -
& 53.5~\cite{cap12}
& 99.8~\cite{cap12} 
& \textbf{97.9}~\cite{speech_commandssota} 
& 74.2~\cite{cap12} 
& 2.5~\cite{cap12} 
& 54.5~\cite{cap12}
& 88.2~\cite{cap12} 
& 79.2~\cite{cap12}
\\
\midrule
\textbf{CAP12} \\
% Architecture avg test voxceleb voxforge speechcommands maskchallenge asvspoof euphonia cremad iemocap params size 
\quad (full)  & \scriptsize{Conformer}
& 606 & 2,200 & 2.99 & 51.0  & 99.7      & 97.1 & 69.2 & 2.5 & 51.3  & 88.2 & 75.5  \\
\quad (3sec) & \scriptsize{Conformer}
& 606 & 2,200 & 2.93 & 47.9  & 99.4      & 97.1 & 69.2 & 3.8 & 49.8  & 88.1 & 74.3    \\
\quad (2sec) & \scriptsize{Conformer}
& 606 & 2,200 & 2.80 & 47.8  & 99.4      & 97.1 & 69.2 & 6.9 & 49.5  & 85.3 & 72.7   \\
\midrule
\textbf{Public} \\
\textbf{Baselines} \\
\quad Wav2Vec2  & Transformer 
& ? & ? & ? & ? & ? & ? & ? & ? & ? & ? & ? \\
\quad TRILL     & Resnetish 
& 24.5 & 86.6 & 1.89 & 13.8 & 84.5 & 77.6 & 65.3 & 6.3 & 47.0 & 65.7 & 55.4 \\
\quad YAMNet     & Resnetish
& 3.7 & 17 & 1.79 & 9.6 & 79.8 & 78.5 & 59.4 & 6.7 & 43.8 & 66.4 & 57.5 \\
\midrule
\textbf{TRILLsson} \\
% voxceleb voxforge speechcommands maskchallenge asvspoof euphonia cremad iemocap 
\quad 5 (2sec) & \scriptsize{AST} % ast_sec3_l12_m2048,48000,tr=False
& 88.7 & 340 & 77.0 & 45.9 & 99.7 & 93.8 & 71.6 & 3.6 & 50.1 & 85.5 & 71.4  \\
\quad 4 (2sec) & \scriptsize{AST} % ast_sec2_l12_m512,32000,tr=False
& 50.8 & 196 & 76.2 & 45.1 & 99.6 & 94.2 & 70.9 & 5.2 & 48.2 & 85.0 & 70.9    \\
\quad 3 (2sec) & \scriptsize{E.NetV2} % efficientnetv2bS,32000,tr=False	
& 21.4 & 95 & 75.2 & 37.9 & 99.3 & 94.8 & 70.9 & 4.1 & 48.4 & 85.0 & 69.0    \\
\quad 2 (2sec) & \scriptsize{E.Net} % efficientnetb3,32000,tr=False	
& 12.2 & 57 & 74.4 & 34.6 & 99.1 & 95.1 & 71.6 & 4.1 & 48.2 & 84.1 & 68.5    \\
\quad 1 (2sec) & \scriptsize{Resnetish} % resnetish_sec3_2352_0.5,48000,tr=False
& 5.0 & 22 & 73.3 & 33.4 & 98.7 & 92.9 & 69.1 & 4.8 & 47.7 & 81.5 & 67.7    \\
\quad 0 (2sec) & \scriptsize{Resnetish} % resnetish_sec3_2352_0.25,48000,tr=False	
& 1.2 & 6.4 & 70.7 & 28.0 & 96.6 & 90.5 & 66.8 & 4.9 & 46.5 & 76.2 & 65.8   \\
%\quad 0 & \scriptsize{Resnetish} % resnetish_sec3_2352_0.25,48000,tr=False	
% & 1.2 & 6.4 & 70.7 & 28.0 & 96.6 & 90.5 & 66.8 & 4.9 & 46.5 & 76.2 & 65.8   \\
\bottomrule
\end{tabular}
\vspace{-3mm}
\end{table*}
\end{centering}

==> table_results_v2_euphonia.tex <==
\begin{centering}
\begin{table*}[t]
\scriptsize
\vspace{-0.2cm}
\caption{Test performance on the NOSS Benchmark and extended tasks. 
``Prev. SoTA" are usually domain specific, but all other rows are linear models on time-averaged input. TRILLsson model sizes are shown without frontends.
%``Prev SoTA" are arbitrarily complicated models, but \textbf{all other rows are linear models on time-averaged input}.
$^\dagger$We use a filtered subset of Voxceleb1 according to YouTube’s privacy guidelines. We omit previous SoTA results on this dataset, since they used the entire dataset.
$^{**}$ASVSpoof uses equal error rate~\cite{asvspoof}. We report the best single-model performance (as compared to model ensembles).
$^{\#}$Euphonia is the only non-public dataset. We use a larger dataset than was reported on in~\cite{cap12}.
$^*$We use the public Wav2Vec 2.0 model from \href{https://huggingface.co/docs/transformers/model_doc/wav2vec2}{Hugging Face}~\cite{transformers_lib}
}\label{tab:results}

\centering
\begin{tabular}{@{} llcc|cccccccc @{}}
\toprule[2pt]
\begin{tabular}{@{}c@{}}Model\\(input size)\end{tabular} &
%Arch. &
\begin{tabular}{@{}c@{}}Params\\ (M)\end{tabular} &
\begin{tabular}{@{}c@{}}Size\\ (MB)\end{tabular} &
Public &
\begin{tabular}{@{}c@{}}Avg D-\\Prime\end{tabular}   & 
Voxceleb1$^\dagger$ & 
Voxforge & 
\begin{tabular}{@{}c@{}}Speech \\ Commands\end{tabular}   &  
\begin{tabular}{@{}c@{}}ASVSpoof\\ 2019$^{**}$\end{tabular} & 
Euphonia$^{\#}$ &
CREMA-D &
IEMOCAP
\\
\toprule[2pt]
\textbf{Prev. SoTA}
& -
& -
& -
& -
%& -
& -
& 99.8~\cite{cap12} 
& 97.9~\cite{speech_commandssota} 
& 2.5~\cite{cap12} 
& -
& 88.2~\cite{cap12} 
& 79.2~\cite{cap12}
\\
\midrule
\textbf{CAP12} \\
% Architecture avg test voxceleb voxforge speechcommands asvspoof euphonia cremad iemocap params size 
\quad (full)  
& 606 & 2,200 & \xmark
& 3.31
& 51.0  & 99.7      & 97.1 & 2.5 & 46.9  & 88.2 & 75.5  \\
\quad (3s) 
& 606 & 2,200 & \xmark
& 3.25
& 47.9  & 99.4      & 97.1 & 3.8 & 46.9  & 88.1 & 74.3    \\
\quad (2s) 
& 606 & 2,200 & \xmark
& 3.10
& 48.1  & 99.4      & 97.0 & 6.9 & 46.9  & 85.3 & 72.7   \\
\midrule
\midrule
\textbf{Baselines} \\
%\quad \begin{tabular}{@{}c@{}}Wav2Vec2*\\(full)\end{tabular} & Transformer
%\quad Wav2Vec2 Lg L6$^*$
%& \tiny{Transformer}
%& ? & ? & \cmark
%& ?
%& ? & ? & ? & ? & ? & ? & ? \\
%\quad Wav2Vec2 Lg. final
%& \tiny{Transformer}
%& ? & ? & \cmark
%& ?
%& ? & ? & ? & ? & ? & ? & ? \\
\quad Wav2Vec2 Sm. L6$^*$
& 93.4 & 360 & \cmark
& ?
& 17.9 & 98.5 & \textbf{95.0} & 6.7 & 48.2 & 77.4 & 65.8 \\
\quad Wav2Vec2 Sm.$^*$
& 93.4 & 360 & \cmark
& ?
& 1.7 & 95.9 & 89.3 & 11.2 & 50.0 & 58.0 & 52.4 \\
\quad TRILL 
%& \tiny{Resnetish}
& 24.5 & 87 & \cmark
& 2.08
& 13.8 & 84.5 & 77.6 & 6.3 & 47.0 & 65.7 & 55.4 \\
%\quad FRILL (1s)     & MobileNet
%& 10 & 36 & \cmark
%& 1.97 & 13.8 & 78.8 & 74.3 & 7.8 & 46.2 & 71.3 & 59.9 \\
\quad YAMNet
%& \tiny{Resnetish}
& 3.7 & 17 & \cmark
& 2.01
& 9.6 & 79.8 & 78.5 & 6.7 & 43.8 & 66.4 & 57.5 \\
\midrule
\textbf{TRILLsson} \\
% voxceleb voxforge speechcommands asvspoof euphonia cremad iemocap 

% ast_sec2_l24_m2048,	678.0	0.447263	0.995385	0.936810	0.071780	0.482906	0.856684	0.712329	
\quad 5 (AST) 
%& \tiny{AST}
& ? & 678 & \cmark
& ?
& \textbf{44.7} & \textbf{99.5} & 93.7 & \textbf{?} & \textbf{48.3} & 85.7 & \textbf{71.2}  \\

% ast_sec2_l24_m512,	390.0	0.429907	0.995418	0.932106	0.090685	0.459984	0.857969	0.709106
\quad 4 (AST) 
& ? & 390 & \cmark
& ?
& 43.0 & \textbf{99.5} & 93.2 & ? & 46.0 & \textbf{85.8} & 70.9    \\

% efficientnetv2bM,	231.0	0.409880	0.991940	0.937219	0.071112	0.480963	0.837404	0.705077
\quad 3 (EffNetv2) 
& ? & 231 & \cmark
& ?
& 41.0 & 99.2 & 93.7 & ? & 48.1 & 83.7 & 70.5    \\

% efficientnetv2b1,	42.0	0.375167	0.991873	0.920654	0.065784	0.445610	0.825835	0.697824
\quad 2 (EffNetv2) 
& ? & 42 & \cmark
& ?
& 37.5 & 99.2 & 92.1 & ? & 44.6 & 82.6 & 69.8    \\

% resnetish_sec2_2352_0.5,	22.0	0.299065	0.978563	0.890798	0.130392	0.458819	0.795630	0.670427
\quad 1 (ResNet) 
& 5.0 & 22 & \cmark
& ?
& 30.0 & 97.9 & 89.1 & ? & 45.9 & 79.6 & 67.0    \\
\bottomrule
\end{tabular}
\vspace{-3mm}
\end{table*}
\end{centering}

==> table_results_v2_noeuphonia.tex <==
\begin{centering}
\begin{table*}[t]
\scriptsize
\vspace{-0.2cm}
\caption{Test performance on the NOSS Benchmark and extended tasks. 
``Prev. SoTA" are usually domain specific, but all other rows are linear models on time-averaged input. TRILLsson model sizes are shown without frontends.
%``Prev SoTA" are arbitrarily complicated models, but \textbf{all other rows are linear models on time-averaged input}.
$^\dagger$We use a filtered subset of Voxceleb1 according to YouTube’s privacy guidelines. We omit previous SoTA results on this dataset, since they used the entire dataset.
$^{**}$ASVSpoof uses equal error rate~\cite{asvspoof}. We report the best single-model performance (as compared to model ensembles).
$^*$We use the public Wav2Vec 2.0 model from \href{https://huggingface.co/docs/transformers/model_doc/wav2vec2}{Hugging Face}~\cite{transformers_lib}
}\label{tab:results}

\centering
\begin{tabular}{@{} llcc|ccccccc @{}}
\toprule[2pt]
\begin{tabular}{@{}c@{}}Model\\(input size)\end{tabular} &
%Arch. &
\begin{tabular}{@{}c@{}}Params\\ (M)\end{tabular} &
\begin{tabular}{@{}c@{}}Size\\ (MB)\end{tabular} &
Public &
\begin{tabular}{@{}c@{}}Avg D-\\Prime\end{tabular}   & 
Voxceleb1$^\dagger$ & 
Voxforge & 
\begin{tabular}{@{}c@{}}Speech \\ Commands\end{tabular}   &  
\begin{tabular}{@{}c@{}}ASVSpoof\\ 2019$^{**}$\end{tabular} &
CREMA-D &
IEMOCAP
\\
\toprule[2pt]
\textbf{Prev. SoTA}
& -
& -
& -
& -
%& -
& -
& 99.8~\cite{cap12} 
& 97.9~\cite{speech_commandssota} 
& 2.5~\cite{cap12} 
& 88.2~\cite{cap12} 
& 79.2~\cite{cap12}
\\
\midrule
\textbf{CAP12} \\
% Architecture avg test voxceleb voxforge speechcommands asvspoof euphonia cremad iemocap params size 
\quad (full)  
& 606 & 2,200 & \xmark
& 3.31
& 51.0  & 99.7      & 97.1 & 2.5  & 88.2 & 75.5  \\
\quad (3s) 
& 606 & 2,200 & \xmark
& 3.25
& 47.9  & 99.4      & 97.1 & 3.8  & 88.1 & 74.3    \\
\quad (2s) 
& 606 & 2,200 & \xmark
& 3.10
& 48.1  & 99.4      & 97.0 & 6.9  & 85.3 & 72.7   \\
\midrule
\midrule
\textbf{Baselines} \\
%\quad \begin{tabular}{@{}c@{}}Wav2Vec2*\\(full)\end{tabular} & Transformer
%\quad Wav2Vec2 Lg L6$^*$
%& \tiny{Transformer}
%& ? & ? & \cmark
%& ?
%& ? & ? & ? & ? & ? & ? & ? \\
%\quad Wav2Vec2 Lg. final
%& \tiny{Transformer}
%& ? & ? & \cmark
%& ?
%& ? & ? & ? & ? & ? & ? & ? \\
\quad Wav2Vec2 Sm. L6$^*$
& 93.4 & 360 & \cmark
& ?
& 17.9 & 98.5 & \textbf{95.0} & 6.7 & 77.4 & 65.8 \\
\quad Wav2Vec2 Sm.$^*$
& 93.4 & 360 & \cmark
& ?
& 1.7 & 95.9 & 89.3 & 11.2 & 58.0 & 52.4 \\
\quad TRILL 
%& \tiny{Resnetish}
& 24.5 & 87 & \cmark
& 2.08
& 13.8 & 84.5 & 77.6 & 6.3 & 65.7 & 55.4 \\
\quad YAMNet
%& \tiny{Resnetish}
& 3.7 & 17 & \cmark
& 2.01
& 9.6 & 79.8 & 78.5 & 6.7 & 66.4 & 57.5 \\
\midrule
\textbf{TRILLsson} \\
% voxceleb voxforge speechcommands asvspoof euphonia cremad iemocap 

% ast_sec2_l24_m2048,	678.0	0.447263	0.995385	0.936810	0.071780	0.482906	0.856684	0.712329	
\quad 5 (AST) 
%& \tiny{AST}
& ? & 678 & \cmark
& ?
& \textbf{44.7} & \textbf{99.5} & 93.7 & \textbf{?} & 85.7 & \textbf{71.2}  \\

% ast_sec2_l24_m512,	390.0	0.429907	0.995418	0.932106	0.090685	0.459984	0.857969	0.709106
\quad 4 (AST) 
& ? & 390 & \cmark
& ?
& 43.0 & \textbf{99.5} & 93.2 & ? & \textbf{85.8} & 70.9    \\

% efficientnetv2bM,	231.0	0.409880	0.991940	0.937219	0.071112	0.480963	0.837404	0.705077
\quad 3 (EffNetv2) 
& ? & 231 & \cmark
& ?
& 41.0 & 99.2 & 93.7 & ? & 83.7 & 70.5    \\

% efficientnetv2b1,	42.0	0.375167	0.991873	0.920654	0.065784	0.445610	0.825835	0.697824
\quad 2 (EffNetv2) 
& ? & 42 & \cmark
& ?
& 37.5 & 99.2 & 92.1 & ? & 82.6 & 69.8    \\

% resnetish_sec2_2352_0.5,	22.0	0.299065	0.978563	0.890798	0.130392	0.458819	0.795630	0.670427
\quad 1 (ResNet) 
& 5.0 & 22 & \cmark
& ?
& 30.0 & 97.9 & 89.1 & ? & 79.6 & 67.0    \\
\bottomrule
\end{tabular}
\vspace{-3mm}
\end{table*}
\end{centering}
